Efficient computation of the Knowledge Gradient for Bayesian Optimization

Bayesian optimization is a powerful collection of methods for optimizing stochastic expensive black box functions. One key component of a Bayesian optimization algorithm is the acquisition function that determines which solution should be evaluated in every iteration. A popular and very effective choice is the Knowledge Gradient acquisition function, however there is no analytical way to compute it. Several different implementations make different approximations. In this paper, we review and compare the spectrum of Knowledge Gradient implementations and propose One-shot Hybrid KG, a new approach that combines several of the previously proposed ideas and is cheap to compute as well as powerful and efficient. We prove the new method preserves theoretical properties of previous methods and empirically show the drastically reduced computational overhead with equal or improved performance. All experiments are implemented in BOTorch and code is available on github.

==> Sections/old_docs/litrev.tex <==
\section{Related Work} \label{sec:related_work}

Bayesian optimization (BO) has gained wide popularity, especially for problems involving expensive black-box functions. BO constructs a surrogate model, usually a Gaussian process (GP) after collecting some initial data. Then, it iteratively uses an acquisition function to decide what data would be most valuable to collect next, explicitly balancing exploration (collecting more information about yet unexplored areas) and exploitation (evaluating solutions that are predicted to be good). After sampling the next solution, the Gaussian process model is updated with the new information and the process is repeated until the available budget of evaluations has been consumed. For a comprehensive introduction see \cite{frazier2018tutorial} and \cite{deFreitas2016}. 

% Deterministic and single objective acquisition functions
Several acquisition functions have been proposed in the literature for single objective problems. The most popular is Expected Improvement (EI) of \cite{jones1998efficient} that measures the expected amount that a new output $f(x)$ improves over the current best sampled design output. \cite{srinivas2010} proposes to optimize an optimistic upper-confidence bound (UCB) acquisition function where the benefit each point $x$ is quantified using a quantile of the distribution $f(x)$. Thompson sampling (TS) \cite{Thompson1933} is a randomized strategy which samples a reward function from the posterior and selects the arm with the highest simulated reward. However, in a continuous design space, TS corresponds to sampling the objective function from the GP posterior and then obtain the sample that maximizes this GP realization. This acquisition function is simple to implement and may be applied for noisy objective functions. \cite{Hernandez-Lobato2014} considers an information-based acquisition function where a GP over outputs generates a distribution over the input domain that models the probability of any input being the maximizer. This acquisition criterion involves computing the expected entropy reduction of the global solution and may be used for noisy observations. 

% KG Literature Review
The Knowledge Gradient (KG) acquisition function (\cite{frazier2009knowledge}) is another myopic acquisition function that aims to maximize the new GP predicted optimal performance after one new sample. KG is derived by reconsidering the assumption made EI where the Bayesian optimization algorithm returns only a previously evaluated design as a final solution. This can be considered as a sensible assumption if the decision maker is highly risk-averse and evaluations are noise-free, but if the decision-maker is willing to tolerate some risk then we may report a design that has uncertainty attached to it. Moreover, if evaluations have noise then, the final recommended solution is necessarily uncertain and any returned solution would require a substantial amount of re-evaluations to determine the quality. Therefore, KG replaces this assumption by allowing the algorithm to return any solution according to the GP predicted performance, even if it has not been previously evaluated.

Although KG has demonstrated superior empirical performance compared to other acquisition functions (\cite{Picheny2013}), especially for larger levels of noise, KG is not available in closed-form. Therefore, many different approximations have been proposed. \cite{frazier2009knowledge} propose discretising the design space and solving a series of linear problems.
% However, increasing the number of dimensions requires more discretization points and thus renders this approach scales poorly in higher dimensions. 
A more recent approach involves Monte-Carlo sampling of the observed value at design $x^{n+1}$, and solving a inner optimization problem for each sample to identify the best posterior mean \cite{wu2017discretization}. 
% Using Monte-Carlo samples improves the scalability of the algorithm in terms of number of dimensions, but the inner optimization still leads to high computational complexity.
\cite{pearce2020practical} proposed a hybrid between between both approaches that consists of obtaining high value points from the predictive posterior GP mean that would serve as a discretization. Combining both approaches allows to leverage  the scalability of the Monte-Carlo based acquisition function and the computational performance of discretising the design space. Lastly, the "one-shot" formulation (\cite{balandat2020botorch}) treats optimizing KG as a deterministic optimization problem. It involves drawing fixed base samples for the inner optimization inside the expectation. Then, the discretization, and the sample decision are jointly optimized. In the end, the sample decision is recommended and the discretization is discarded as an optimization by-product.

% Contribution (?)
EI, UCB are fast but simple. KG,. ES, MES are slow yet more advanced. WE propose hybrid KG that is both fast and sophisticated.
{\bf I think we'll never be able to compete with EI and UCB in terms of speed. So may have to word more carefully.}


% Single Objective acquisition functions
% \begin{itemize}
    % \item Efficient Global Optimisation (EGO) algorithm of 
    
    % \item \cite{Letham2017} extended Expected Improvement to noisy observations (NEI) by iterating the expectation over possible posterior distributions.
    
    % \item In contrast to the improvement-based acquisition functions introduced so far, \cite{srinivas2010} proposes to optimise an optimistic upper-confidence bound (UCB) acquisition function where the benefit each point $x$ is quantified using a quantile of the distribution $f(x)$.
    
    
    % \item \cite{Hernandez-Lobato2014} considers an information-based acquisition function where a GP over outputs generates a distribution over the input domain that models the probability of any input being the maximiser. This acquisition criterion involves computing the expected entropy reduction of the global solution and may be used for noisy observations. 
    
    % \item Thompson sampling (TS) \cite{Thompson1933} is a randomised strategy which samples a reward function from the posterior and selects the arm with the highest simulated reward. However, in a continuous design space, TS corresponds to sampling the objective function from the GP posterior and then obtain the sample that maximises this GP realisation. This acquisition function is simple to implement and may be applied for noisy objective functions.
% \end{itemize}

% KG specific implementations

% \begin{itemize}

%     \item \cite{Picheny2013} showed that KG is empirically superior, especially for larger levels of noise.
    
%     \item  KG: The Knowledge Gradient (KG) policy for Continuous Parameters (\citeauthor{Frazier2009} \citeyear{Frazier2009}) is another myopic acquisition function that aims to maximise the new predicted optimal performance after one new sample. Different from EGO, KG accounts for covariance when judging the value of a sample and can be directly applied to noisy functions.
    
%     \item Discrete KG: \cite{frazier2009knowledge} propose discretising the design space and solving a series of linear problems. However, increasing the number of dimensions requires more discretisation points and thus renders this approach scales poorly in higher dimensions. 
    
%     \item Monte Carlo KG: A more recent approach involves Monte-Carlo sampling of the observed value at design $x^{n+1}$, and solving a inner optimisation problem for each sample to identify the best posterior mean \cite{wu2017discretization}. Using Monte-Carlo samples improves the scalability of the algorithm in terms of number of dimensions, but the inner optimisation still leads to high computational complexity. 
    
%     \item HYBRIDKG \cite{pearce2020practical} propose a hybrid between between both approaches that consists of obtaining high value points from the predictive posterior GP mean that would serve as a discretisation. Combining both approaches allows to leverage  the scalability of the Monte-Carlo based acquisition function and the computational performance of discretising the design space.
    
%     \item ONESHOT The "one-shot" formulation treats optimizing KG as a deterministic optimisation problem. It involves drawing fixed base samples for the inner optimisation inside the expectation. Then, the discretisation, $X_{d}$, and the sample decision $x^{n+1}=x$ are jointly optimised. In the end, the sample decision is recommended and the discretisation is discarded as an optimisation by-product.
    
% \end{itemize}



==> Sections/todo.tex <==
\noindent\Michael{
TODO
\begin{itemize}
    \item proofs
    \item (optional with Juan) step-by-step hybrid OS KG figure
    \item extra material in the appendix
    \item read end-to-end
    \item blog post + animations + link in abstract
\end{itemize}
}

\noindent\Juan{
TODO
\begin{itemize}
    \item (optional with Juan) step-by-step hybrid OS KG figure
    \item read end-to-end
    \item main paper: log(wall clock) vs log(OC), cherry pick illustrative plots
    \begin{itemize}
        \item OS KG 3, 512
        \item H KG 3, 10
        \item OSH KG 3, 10
    \end{itemize}
    \item One single iterations, one set of points, one GP, true KG value over time estimated by standard hybrid KG
    \item sensitivity analysis
    \item optimise some instances, test on others
    \item how do optimal parameters depend on lengthscale and iteration number?
    \item Parameter tuning is actually a MO problem - time vs. quality
    \item Appendix: log(wall clock) vs log(OC) aaalllll plots
    \item (optional) open source code + README.md with instructions to reproduce
\end{itemize}
}
